GaussianHeads: End-to-End Learning of Drivable Gaussian Head Avatars from Coarse-to-fine Representations

Real-time rendering of human head avatars is a cornerstone of many computer graphics applications, such as augmented reality, video games, and films, to name a few. Recent approaches address this challenge with computationally efficient geometry primitives in a carefully calibrated multi-view setup. Albeit producing photorealistic head renderings, it often fails to represent complex motion changes such as the mouth interior and strongly varying head poses. We propose a new method to generate highly dynamic and deformable human head avatars from multi-view imagery in real-time. At the core of our method is a hierarchical representation of head models that allows to capture the complex dynamics of facial expressions and head movements. First, with rich facial features extracted from raw input frames, we learn to deform the coarse facial geometry of the template mesh. We then initialize 3D Gaussians on the deformed surface and refine their positions in a fine step. We train this coarse-to-fine facial avatar model along with the head pose as a learnable parameter in an end-to-end framework. This enables not only controllable facial animation via video inputs, but also high-fidelity novel view synthesis of challenging facial expressions, such as tongue deformations and fine-grained teeth structure under large motion changes. Moreover, it encourages the learned head avatar to generalize towards new facial expressions and head poses at inference time. We demonstrate the performance of our method with comparisons against the related methods on different datasets, spanning challenging facial expression sequences across multiple identities. We also show the potential application of our approach by demonstrating a cross-identity facial performance transfer application.

==> sections/disccusions.tex <==
\section{Limitations and Future Work} \label{sec:discussions}


Our method produces photorealistic renderings of human heads and large deformations at high speed. Nevertheless, a few limitations exist that are up to future works to address. First, our framework is supervised by per-frame mesh tracking of multi-view RGB images, and inaccurate initial tracking results could lead to poor rendering performance. Future approaches can investigate image-based supervision and/or a temporal attention mechanism to improve the robustness to tracking and temporal consistency. Second, our coarse 3D head model does not explicitly include hair~\cite{li2017_flame}. We believe that introducing a hair dynamics model akin to NeuWigs\cite{Wang_2023_CVPR} will allow for better rendering of hair dynamics. Driving our model from an in-the-wild setup is also an interesting future direction, as it paves the way to lightweight mobile systems such as VR headsets or Egocentric hardware \cite{EgoChat20}.  



==> sections/tongue.tex <==
\begin{figure}[]
	\centering
    \includegraphics[width=\linewidth]{figures_main/method_suipporting.drawio.png}
	\caption{\textbf{Coarse-to-fine Learning.} We refine the FLAME shape-fitted mesh by an initial registration step (b), which results in the template mesh with vertices $v_t$ used in our framework. (c) The template mesh is deformed based on the input and posed to the world space using the global transformation parameters. We initialize the 3D Gaussians on the rigidly translated deformed mesh with vertices and refine their properties through our Coarse-to-Fine framework, resulting in dense, head surface-aligned 3D Gaussians (d). The 3D Gaussians are splatted, resulting in the render (e), which is supervised with ground truth image (f). 
  }
	\label{fig:intermediates}
\end{figure}

